DexterCap: An Affordable and Automated System for Capturing Dexterous Hand-Object Manipulation

Capturing fine-grained hand-object interactions is challenging due to severe self-occlusion from closely spaced fingers and the subtlety of in-hand manipulation motions. Existing optical motion capture systems rely on expensive camera setups and extensive manual post-processing, while low-cost vision-based methods often suffer from reduced accuracy and reliability under occlusion. To address these challenges, we present DexterCap, a low-cost optical capture system for dexterous in-hand manipulation. DexterCap uses dense, character-coded marker patches to achieve robust tracking under severe self-occlusion, together with an automated reconstruction pipeline that requires minimal manual effort. With DexterCap, we introduce DexterHand, a dataset of fine-grained hand-object interactions covering diverse manipulation behaviors and objects, from simple primitives to complex articulated objects such as a Rubik's Cube. We release the dataset and code to support future research on dexterous hand-object interaction. Project website: https://pku-mocca.github.io/Dextercap-Page/

==> sections/0_abstract.tex <==


\begin{abstract}

Modeling complex, fine-grained hand-object interactions remains challenging, in part due to the limited availability of dedicated datasets and specialized capture methods. Existing motion capture systems are generally limited to basic motion types, such as grasping, and interactions with primitive rigid or articulated objects. To facilitate the exploration of intricate, dexterous in-hand manipulations with more complex objects, we present DexterCap. We first design a robust, low-cost, and high-fidelity motion capture hardware system that acquires reliable data even in the presence of self-occlusion and complex manipulation. To ensure accurate capture despite severe occlusions, we introduce a specialized patch maker equipped with an effective detection and optimization pipeline. We further develop an automated data augmentation pipeline to reconstruct and refine motion data with minimal manual effort, improving both efficiency and data quality. Using this system, we create the DexterHand dataset, which includes subtle, fine-grained manipulation behaviors and interactions with multi-jointed objects such as a Rubik’s cube. By releasing the dataset and supporting source code to the community, we hope that DexterCap will facilitate further research on intricate hand-object interactions.

\end{abstract}

\keywords{Hand-Object Interaction, Motion Capture, Dataset, Animation}



==> sections/0_authors.tex <==

% Authors.
%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
% \author{Heyuan Yao}
% \email{heyuanyao@pku.edu.cn}
% \orcid{0000-0002-6168-6777}
% \affiliation{%
%   \institution{School of Computer Science, Peking University}
%   \streetaddress{No.5 Yiheyuan Road, Haidian District}
%   \city{Beijing}
%   % \state{Beijing}
%   \country{China}
%   \postcode{100871}
% }


% \author{Libin Liu}
% \authornote{corresponding author}
% \email{libin.liu@pku.edu.cn}
% \orcid{0000-0003-2280-6817}
% \affiliation{%
%   \institution{Peking University}
%   \streetaddress{No.5 Yiheyuan Road, Haidian District}
%   \city{Beijing}
%   % \state{Beijing}
%   \country{China}
%   \postcode{100871}
% }
% \affiliation{%
%   \institution{State Key Lab of General AI}
%   \streetaddress{No.5 Yiheyuan Road, Haidian District}
%   \city{Beijing}
%   % \state{Beijing}
%   \country{China}
%   \postcode{100871}
% }
%School of Computer Science and Key Laboratory of Machine Perception (MOE)
%School of Artificial Intelligence and Key Laboratory of Machine Perception (MOE)
% This command defines the author string for running heads.
%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.


% \renewcommand{\shortauthors}{DeJohnette, Rowland-Smith, Badeeri, and Foyt}



% DO NOT ENTER AUTHOR INFORMATION FOR ANONYMOUS TECHNICAL PAPER SUBMISSIONS TO SIGGRAPH 2019!
%\author{Gang Zhou}
%\orcid{1234-5678-9012-3456}
%\affiliation{%
%  \institution{College of William and Mary}
%  \streetaddress{104 Jamestown Rd}
%  \city{Williamsburg}
%  \state{VA}
%  \postcode{23185}
%  \country{USA}}
%\email{gang_zhou@wm.edu}
%\author{Valerie B\'eranger}
%\affiliation{%
%  \institution{Inria Paris-Rocquencourt}
%  \city{Rocquencourt}
%  \country{France}
%}
%\email{beranger@inria.fr}
%\author{Aparna Patel}
%\affiliation{%
% \institution{Rajiv Gandhi University}
% \streetaddress{Rono-Hills}
% \city{Doimukh}
% \state{Arunachal Pradesh}
% \country{India}}
%\email{aprna_patel@rguhs.ac.in}
%\author{Huifen Chan}
%\affiliation{%
%  \institution{Tsinghua University}
%  \streetaddress{30 Shuangqing Rd}
%  \city{Haidian Qu}
%  \state{Beijing Shi}
%  \country{China}
%}
%\email{chan0345@tsinghua.edu.cn}
%\author{Ting Yan}
%\affiliation{%
%  \institution{Eaton Innovation Center}
%  \city{Prague}
%  \country{Czech Republic}}
%\email{yanting02@gmail.com}
%\author{Tian He}
%\affiliation{%
%  \institution{University of Virginia}
%  \department{School of Engineering}
%  \city{Charlottesville}
%  \state{VA}
%  \postcode{22903}
%  \country{USA}
%}
%\affiliation{%
%  \institution{University of Minnesota}
%  \country{USA}}
%\email{tinghe@uva.edu}
%\author{Chengdu Huang}
%\author{John A. Stankovic}
%\author{Tarek F. Abdelzaher}
%\affiliation{%
%  \institution{University of Virginia}
%  \department{School of Engineering}
%  \city{Charlottesville}
%  \state{VA}
%  \postcode{22903}
%  \country{USA}
%}

%\renewcommand\shortauthors{Zhou, G. et al}

==> sections/0_teaser.tex <==
% A "teaser" figure, centered below the title and authors and above the body of the work.

\begin{teaserfigure}
    \centering
    \includegraphics[width=0.9\linewidth]{figures/teaser/comparison_result-no_bg-arrow.png}
    \caption{DexterCap capturing Rubik's cube manipulation. Top row: raw multi-camera footage with character-coded checkerboard markers enabling reliable tracking despite complex occlusions. Bottom row: reconstructed 3D hand and object motion. Our markers capture detailed motion while preserving natural manipulation dynamics.}
\end{teaserfigure}


==> sections/_template_args.tex <==

%% NOTE that a single column version may be required for 
%% submission and peer review. This can be done by changing
%% the \doucmentclass[...]{acmart} in this template to 
%% \documentclass[manuscript,screen]{acmart}
%% 
%% To ensure 100% compatibility, please check the white list of
%% approved LaTeX packages to be used with the Master Article Template at
%% https://www.acm.org/publications/taps/whitelist-of-latex-packages 
%% before creating your document. The white list page provides 
%% information on how to submit additional LaTeX packages for 
%% review and adoption.
%% Fonts used in the template cannot be substituted; margin 
%% adjustments are not allowed.
%%
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2022}
%\acmYear{2022}
%\acmDOI{10.1145/1122445.1122456}

% \setcopyright{acmlicensed}
\acmJournal{TOG}
% \acmYear{2024} 
% \acmVolume{43} 
% \acmNumber{4} 
% \acmArticle{144} 
% \acmMonth{7}
% \acmDOI{10.1145/3658137}

%% These commands are for a PROCEEDINGS abstract or paper.
%\acmConference[SIGGRAPH '22]{SIGGRAPH 2022}{June 03--05, 2021}{Virtual Event}
%% \acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%% June 03--05, 2018, Woodstock, NY}
%\acmPrice{15.00}
%\acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
% \acmSubmissionID{247}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
\citestyle{acmauthoryear}
%\setcitestyle{nosort,square} % nosort to allow for manual chronological ordering

% A useful command for controlling the number of authors per row.
% The default value of "authorsperrow" is 2.
% \settopmatter{authorsperrow=4}
